TerraWatt: Sustaining Sustainable Computing of Containers in Containers

Each day the world inches closer to a climate catastrophe and a sustainability revolution. To avoid the former and achieve the latter we must transform our use of energy. Surprisingly, today's growing problem is that there is too much wind and solar power generation at the wrong times and in the wrong places. We argue for the construction of TerraWatt: a geographically-distributed, large-scale, zero-carbon compute infrastructure using renewable energy and older hardware. Delivering zero-carbon compute for general cloud workloads is challenging due to spatiotemporal power variability. We describe the systems challenges in using intermittent renewable power at scale to fuel such an older, decentralized compute infrastructure.

==> extra.tex <==
\section{Extra/old stuff}

\paragraph{Abstractions and infrastructure:} Modern cloud abstractions for compute and storage are familiar to developers and have been refined over time. However such abstractions, and the infrastructure that backs them, were never designed for spatially-fragmented compute running on heterogenous, older infrastructure with uncertain and intermittent power availability. The nature of these new constraints requires wholesale re-evaluation and possibly redesign of the cloud for the zero-carbon era.

\paragraph{Legacy compute:} The form factor we consider is one of old shipping containers filled with old computers that were otherwise likely to be scrapped, set up as self-sufficient compute that will be used only as the energy metric dictates. To achieve this we must perform scheduling of three elements: location (where the containers are physically located so as to tap into renewable energy), power (when to run the compute so as to use opportunity power), and jobs (which jobs to run in which containers in containers). These factors place requirements on the abstractions and infrastructure we develop.

\paragraph{Metrics.} In this paper we introduce a new metric for sustainable computing:  \emph{energy/flops}, which captures the full energetic footprint of each unit of compute.  Using this metric, we explore how both renewable energy generation (which decreases the ecological footprint of the electricity consumed) and repurposed old hardware (which decreases the ecological footprint of the physical machines) can be combined to yield computing that is of the lowest impact that we know of to date. We then discuss how such compute can be made practical and deployable at scale, accounting for all relevant costs (both monetary and energetic).


\subsection{Notes from discussion}


Notes: Islanding as a concept to mention.  As a sub-part of a discussion of reliability

Is zero carbon renewable cloud really just "spot instances"? Is it the same thing?

Would applying spot instance pricing solve the problem?

Distinction: many tiers of instances

possible thoughts: with 5 minutes warning, can you migrate data/compute away before the power goes away?

can one container be divided into tiers of "spotness". As power goes from 1.0 down to 0.0, could turn off parts in series

Replicate compute: n of K, but K is free anyways

one datacenter network limited to N machines, if you want more than N machines, need to use multiple put together

Distinction between zero-carbon and spot instances: long-term job scheduling because power may not be available

Agenda items:
1. Hotos paper (Feb 3)
2. "Berkeley view" style paper w/ information batteries
3a. Proposal: an infrastructure that would be coming out of these ideas (a mid-scale)
3b. Approach VMware for private funding?

Major question: what makes this look different than the typical cloud?

What systems infrastructure is core vs. left to users? (e.g., migration, etc.)

What are the key compute abstractions?

\subsection{Precomputation and caching}
(gmporter: this seems like it's in the wrong section)
There has been previous work done scheduling compute tasks under a variety of constraints at the cloud and high performance scale. Google recently announced their "carbon-intelligent computing platform" that attempts to reduce carbon emission of datacenters by aligning time-insensitive tasks with periods of high renewable energy availability \cite{google}. In this paper, we will refer to this technique and similar techniques as time-shifted compute.

Memoization is a well known technique used to improve the performance of programs by caching the results of expensive computations for later use. Previous work has been done exploring the profitability of program memoization at the trace level, the basic block level, and the function level \cite{bbmemoize, trace_level_reuse, dynamic_trace_memoization}. In this work, we chose to focus on function level memoization as memoization at finer granularity has typically relied on hardware techniques to be effective .   

Suresh et al. have shown that a subset of functions can be benefit from software memoization performed at compile and load time. These functions share the following characteristics: expensive, side-effect free, critical, and repetitive arguments \cite{ltmemoize}. Using compile time memoization, Suresh et al. were able to achieve modest performance gains on a subset of SPEC benchmarks that contain memoizable functions in the critical paths \cite{ctmemoize}. 

In this work, we apply these memoization techniques to precompute a table of values for memoizable functions that lie in the program's critical path. These tables are then used to improve the runtime of a program at execution.  

==> future-misc.tex <==
\section{Future Work / Misc Text}

\subsection{Networking aspects}
What is the Internet's physical map?

